On Network Functional Compression

In this paper, we consider different aspects of the network functional compression problem where computation of a function (or, some functions) of sources located at certain nodes in a network is desired at receiver(s). The rate region of this problem has been considered in the literature under certain restrictive assumptions, particularly in terms of the network topology, the functions and the characteristics of the sources. In this paper, we present results that significantly relax these assumptions. Firstly, we consider this problem for an arbitrary tree network and asymptotically lossless computation. We show that, for depth one trees with correlated sources, or for general trees with independent sources, a modularized coding scheme based on graph colorings and Slepian-Wolf compression performs arbitrarily closely to rate lower bounds. For a general tree network with independent sources, optimal computation to be performed at intermediate nodes is derived. We introduce a necessary and sufficient condition on graph colorings of any achievable coding scheme, called coloring connectivity condition (C.C.C.). Secondly, we investigate the effect of having several functions at the receiver. In this problem, we derive a rate region and propose a coding scheme based on graph colorings. Thirdly, we consider the functional compression problem with feedback. We show that, in this problem, unlike Slepian-Wolf compression, by having feedback, one may outperform rate bounds of the case without feedback. Fourthly, we investigate functional computation problem with distortion. We compute a rate-distortion region for this problem. Then, we propose a simple suboptimal coding scheme with a non-trivial performance guarantee. Finally, we introduce cases where finding minimum entropy colorings and therefore, optimal coding schemes can be performed in polynomial time.

==> biblio.tex <==
%% This defines the bibliography file (main.bib) and the bibliography style.
%% If you want to create a bibliography file by hand, change the contents of
%% this file to a `thebibliography' environment.  For more information 
%% see section 4.3 of the LaTeX manual.
\begin{singlespace}
\bibliography{main}
\bibliographystyle{plain}
\end{singlespace}


==> distortion1.tex <==

One may note when the number of vertices is small, constructing these graphs is not computationally difficult. Among all $\fh$ which lead to the same $D$-characteristic graphs, one can choose a function which minimizes the distortion.    
\end{comment}
\begin{comment}
\section{Summary of Results}\label{sec:con}

In this section, we considered the problem of functional compression with distortion $D$. In this problem, a deterministic function of some correlated sources is desired at the receiver with distortion $D$. Some work (\cite{doshi-dist} and \cite{yam}) has addressed the side information version of this problem. Here, we considered distributed functional compression. We computed a feasible rate-distortion region and proposed an achievable scheme. For the case $D=0$, our results are simplified to the lossless functional compression's results discussed in Section \ref{chap:tree}.  

\end{comment}

